iDb-A*: Iterative Search and Optimization for Optimal Kinodynamic Motion Planning

Motion planning for robotic systems with complex dynamics is a challenging problem. While recent sampling-based algorithms achieve asymptotic optimality by propagating random control inputs, their empirical convergence rate is often poor, especially in high-dimensional systems such as multirotors. An alternative approach is to first plan with a simplified geometric model and then use trajectory optimization to follow the reference path while accounting for the true dynamics. However, this approach may fail to produce a valid trajectory if the initial guess is not close to a dynamically feasible trajectory. In this paper, we present Iterative Discontinuity Bounded A* (iDb-A*), a novel kinodynamic motion planner that combines search and optimization iteratively. The search step utilizes a finite set of short trajectories (motion primitives) that are interconnected while allowing for a bounded discontinuity between them. The optimization step locally repairs the discontinuities with trajectory optimization. By progressively reducing the allowed discontinuity and incorporating more motion primitives, our algorithm achieves asymptotic optimality with excellent any-time performance. We provide a benchmark of 43 problems across eight different dynamical systems, including different versions of unicycles and multirotors. Compared to state-of-the-art methods, iDb-A* consistently solves more problem instances and finds lower-cost solutions more rapidly.

==> files_tro/merged_2023-10-23--14-55-10.tex.nice.tex <==
\begin{tabular}{lllrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{iDb-A*} & \multicolumn{4}{c}{SST*} & \multicolumn{4}{c}{RRT*+TO}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
 \# & System & Instance & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$\\
\midrule
0 & Acrobot & swing up & \textbf{1.0} & 1.4 & 5.8 & 4.5 & 0.3 & - & - & - & 0.7 & \textbf{0.8} & \textbf{4.0} & \textbf{4.0}\\
1 & Acrobot & swing obstacles 1 & \textbf{1.0} & 2.0 & 6.0 & 5.0 & 0.3 & - & - & - & \textbf{1.0} & \textbf{1.4} & \textbf{5.7} & \textbf{3.7}\\
2 & Car+Trailer & kink & \textbf{1.0} & 1.2 & \textbf{25.6} & \textbf{15.8} & \textbf{1.0} & \textbf{0.8} & 84.0 & 65.1 & \textbf{1.0} & 4.5 & 43.2 & 17.7\\
3 & Car+Trailer & park & \textbf{1.0} & \textbf{0.1} & 7.9 & \textbf{4.2} & 0.7 & 6.4 & 37.6 & 8.9 & 0.8 & 0.3 & \textbf{5.9} & 5.4\\
4 & Planar Rotor & hole & \textbf{1.0} & 12.7 & \textbf{3.6} & \textbf{3.1} & 0.8 & 56.8 & 9.9 & 7.5 & \textbf{1.0} & \textbf{11.7} & 9.8 & 3.6\\
5 & Planar Rotor & bugtrap & \textbf{1.0} & 14.0 & \textbf{5.5} & \textbf{5.0} & 0.9 & 22.0 & 12.7 & 8.7 & \textbf{1.0} & \textbf{2.6} & 13.8 & 8.4\\
6 & Rotor Pole & swing up obstacles & \textbf{1.0} & \textbf{2.2} & \textbf{4.0} & \textbf{3.9} & 0.0 & - & - & - & 0.8 & 49.3 & 5.3 & 4.0\\
7 & Rotor Pole & small window & \textbf{1.0} & \textbf{3.2} & \textbf{4.5} & \textbf{4.5} & 0.0 & - & - & - & 0.3 & - & - & -\\
8 & Quadrotor v0 & recovery & \textbf{1.0} & \textbf{0.8} & \textbf{6.2} & \textbf{2.6} & 0.0 & - & - & - & 0.0 & - & - & -\\
9 & Quadrotor v0 & recovery obstacles & \textbf{1.0} & \textbf{1.3} & \textbf{5.3} & 3.5 & 0.0 & - & - & - & \textbf{1.0} & 6.0 & 6.0 & \textbf{3.3}\\
10 & Quadrotor v1 & obstacle & \textbf{1.0} & \textbf{1.1} & \textbf{2.7} & \textbf{2.4} & 0.1 & - & - & - & \textbf{1.0} & 1.3 & 4.3 & 3.6\\
11 & Quadrotor v1 & window & \textbf{1.0} & 1.5 & \textbf{2.6} & \textbf{2.2} & 0.1 & - & - & - & 0.3 & - & - & -\\
12 & Unicycle 1 v0 & bugtrap & \textbf{1.0} & 0.5 & \textbf{22.6} & \textbf{20.9} & \textbf{1.0} & \textbf{0.1} & 77.8 & 24.0 & \textbf{1.0} & 1.3 & 48.9 & 23.4\\
13 & Unicycle 1 v2 & wall & \textbf{1.0} & 0.7 & \textbf{20.8} & \textbf{18.4} & \textbf{1.0} & \textbf{0.2} & 47.6 & 19.0 & 0.1 & - & - & -\\
14 & Unicycle 2 & bugtrap & \textbf{1.0} & 1.3 & \textbf{25.2} & \textbf{25.0} & \textbf{1.0} & \textbf{0.7} & 99.1 & 45.7 & \textbf{1.0} & 2.8 & 53.0 & 28.4\\
15 & Unicycle 2 & park & \textbf{1.0} & \textbf{0.1} & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.1} & 16.8 & 6.1 & \textbf{1.0} & \textbf{0.1} & 6.0 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp/merged_2023-05-11--17-42-07.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
&  \multicolumn{3}{c}{idba*} & \multicolumn{3}{c}{sst} & \multicolumn{3}{c}{geo}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 & icf & ilc & itf & scf & slc & stf & gcf & glc & gtf \\
\midrule
uni2\_0/kink\_0 & 19.8 & 17.7 & 1.1 & -1.0 & -1.0 & 40.1 & 32.2 & 19.3 & 2.0 \\
uni2\_0/park & 5.8 & 5.8 & 0.2 & -1.0 & -1.0 & 40.1 & 5.9 & 5.9 & 0.3 \\
uni2\_0/bugtrap\_0 & 27.2 & 25.1 & 2.2 & -1.0 & -1.0 & 40.1 & 33.9 & 28.4 & 2.0 \\
uni1\_0/park & 3.4 & 3.3 & 0.2 & 6.1 & 3.3 & 0.1 & 3.2 & 3.1 & 0.2 \\
uni1\_0/bugtrap\_0 & 21.6 & 21.0 & 2.1 & 62.9 & 56.1 & 2.0 & 35.1 & 24.5 & 3.5 \\
uni1\_0/kink\_0 & 21.1 & 13.3 & 1.4 & 49.2 & 32.9 & 0.4 & 25.0 & 14.0 & 1.2 \\
uni1\_1/kink\_0 & 22.6 & 21.1 & 1.2 & -1.0 & -1.0 & 40.1 & 37.4 & 28.4 & 8.1 \\
uni1\_2/wall\_0 & 18.9 & 18.1 & 0.8 & 41.1 & 41.1 & 31.7 & -1.0 & -1.0 & 40.1 \\
car\_first\_order\_with\_1\_trailers\_0/kink\_0 & 16.5 & 16.7 & 4.8 & 59.6 & 58.3 & 9.6 & 39.5 & 35.6 & 13.2 \\
car\_first\_order\_with\_1\_trailers\_0/bugtrap\_0 & 19.0 & 19.0 & 13.7 & 47.1 & 44.4 & 0.6 & -1.0 & -1.0 & 40.1 \\
car\_first\_order\_with\_1\_trailers\_0/park & 4.8 & 4.8 & 1.0 & -1.0 & -1.0 & 40.1 & 6.0 & 6.0 & 1.2 \\
quad2d/empty\_0 & 2.5 & 1.1 & 5.3 & 3.2 & 3.0 & 1.4 & 1.2 & 1.2 & 0.2 \\
quad2d/quad\_obs\_column & 5.3 & 3.6 & 6.8 & -1.0 & -1.0 & 40.1 & 10.1 & 4.0 & 4.8 \\
quad2d/quad2d\_recovery\_wo\_obs & 3.8 & 3.8 & 5.3 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
acrobot/swing\_up\_empty & 4.5 & 4.8 & 8.7 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
acrobot/swing\_down\_easy & 3.3 & 3.1 & 1.2 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
acrobot/swing\_down & 4.1 & 4.0 & 3.8 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
quadrotor\_0/empty\_0\_easy & 2.6 & 2.6 & 3.5 & -1.0 & -1.0 & 40.1 & 0.7 & 0.7 & 0.1 \\
quadrotor\_0/recovery & 2.6 & 2.6 & 5.5 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
quadrotor\_0/quad\_one\_obs & 3.2 & 3.4 & 17.9 & -1.0 & -1.0 & 40.1 & -1.0 & -1.0 & 40.1 \\
\bottomrule
\end{tabular}

==> results_tmp/merged_2023-06-21--14-10-37.tex.nice.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
&  \multicolumn{3}{c}{idba*} & \multicolumn{3}{c}{sst*} & \multicolumn{3}{c}{geo}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& cf & cl & tf & cf & cl & tf & cf & cl & tf \\
\midrule
uni1\_0/park & 3.5 & \textbf{3.1} & 0.2 & 10.0 & 3.2 & \textbf{0.1} & \textbf{3.5} & 3.2 & 0.2\\
uni1\_0/bugtrap\_0 & \textbf{21.9} & \textbf{20.7} & 2.0 & 74.3 & 31.9 & \textbf{1.0} & 31.1 & 23.8 & 5.5\\
uni1\_0/kink\_0 & \textbf{21.5} & \textbf{13.2} & 1.5 & 49.1 & 19.3 & \textbf{0.5} & 24.7 & 13.8 & 2.7\\
uni1\_1/kink\_0 & \textbf{21.3} & \textbf{21.1} & \textbf{1.5} & 40.6 & 26.5 & 13.0 & 32.6 & 23.8 & 5.2\\
uni1\_2/wall\_0 & \textbf{20.0} & \textbf{18.1} & \textbf{1.5} & 45.0 & 28.9 & 4.1 & - & - & -\\
uni2\_0/kink\_0 & \textbf{17.8} & \textbf{17.7} & \textbf{1.2} & 71.3 & 66.4 & 3.4 & 28.9 & 20.6 & 4.2\\
uni2\_0/park & \textbf{5.8} & \textbf{5.8} & \textbf{0.3} & 22.4 & 10.0 & 0.6 & 5.9 & 5.8 & 0.7\\
uni2\_0/bugtrap\_0 & \textbf{26.2} & \textbf{25.1} & \textbf{1.9} & 66.2 & 61.1 & 6.3 & 32.2 & 31.4 & 38.1\\
car\_first\_order\_with\_1\_trailers\_0/kink\_0 & \textbf{24.2} & \textbf{15.1} & \textbf{2.6} & 56.2 & 66.0 & 5.7 & 27.3 & 22.3 & 20.3\\
car\_first\_order\_with\_1\_trailers\_0/bugtrap\_0 & \textbf{22.2} & \textbf{19.0} & \textbf{1.5} & 42.7 & 43.3 & 2.5 & - & - & -\\
car\_first\_order\_with\_1\_trailers\_0/park & 8.4 & \textbf{4.5} & 1.3 & 9.2 & 6.6 & \textbf{0.9} & \textbf{4.9} & 4.9 & 3.1\\
quad2d/empty\_0 & \textbf{1.0} & \textbf{1.0} & 1.0 & 1.5 & 1.3 & 14.3 & 1.0 & 1.0 & \textbf{0.2}\\
quad2d/empty\_1 & \textbf{1.3} & \textbf{1.3} & \textbf{0.6} & 2.3 & 1.9 & 5.6 & 1.4 & 1.4 & 1.1\\
quad2d/quad\_obs\_column & \textbf{3.2} & \textbf{3.1} & \textbf{4.2} & 6.5 & 6.5 & 114.0 & 8.1 & 8.1 & 54.0\\
quad2d/quad\_bugtrap & \textbf{5.2} & \textbf{5.2} & \textbf{7.9} & - & - & - & - & - & -\\
quad2d/quad2d\_recovery\_wo\_obs & \textbf{3.2} & \textbf{3.1} & \textbf{3.7} & - & - & - & - & - & -\\
quad2d/quad2d\_recovery\_obs & \textbf{4.5} & \textbf{4.5} & \textbf{11.6} & - & - & - & - & - & -\\
quad2d/fall\_through & \textbf{4.0} & \textbf{3.1} & \textbf{4.0} & - & - & - & - & - & -\\
quad2dpole/move\_with\_down & 2.4 & 2.4 & \textbf{0.6} & - & - & - & \textbf{2.4} & \textbf{2.4} & 2.6\\
quad2dpole/move\_with\_up & 5.2 & 3.9 & \textbf{1.9} & - & - & - & \textbf{3.1} & \textbf{3.1} & 2.8\\
quad2dpole/up & \textbf{3.8} & \textbf{3.7} & \textbf{7.5} & - & - & - & 4.2 & 4.2 & 9.2\\
quad2dpole/down & \textbf{3.9} & \textbf{3.2} & \textbf{1.5} & - & - & - & 5.7 & 5.7 & 15.8\\
quad2dpole/up\_obs & \textbf{4.0} & \textbf{3.9} & \textbf{4.8} & - & - & - & - & - & -\\
quad2dpole/window\_easy & \textbf{5.0} & \textbf{4.6} & \textbf{31.0} & - & - & - & - & - & -\\
quad2dpole/window & \textbf{4.4} & \textbf{4.3} & \textbf{13.5} & - & - & - & - & - & -\\
quad2dpole/window\_hard & \textbf{4.5} & \textbf{4.5} & \textbf{8.0} & - & - & - & - & - & -\\
acrobot/swing\_up\_empty & 7.9 & 8.2 & \textbf{7.1} & - & - & - & \textbf{3.8} & \textbf{3.6} & 7.6\\
acrobot/swing\_up\_obs & 9.1 & 8.7 & \textbf{7.5} & - & - & - & \textbf{3.7} & \textbf{3.6} & 7.6\\
acrobot/swing\_up\_obs\_hard & 5.2 & 4.9 & 9.5 & - & - & - & \textbf{4.3} & \textbf{3.6} & \textbf{4.8}\\
acrobot/swing\_down\_easy & \textbf{3.6} & \textbf{3.7} & \textbf{2.4} & - & - & - & - & - & -\\
acrobot/swing\_down & 6.4 & 5.7 & 4.8 & - & - & - & \textbf{3.9} & \textbf{3.6} & \textbf{3.5}\\
quadrotor\_0/empty\_0\_easy & 1.3 & 1.3 & \textbf{0.5} & - & - & - & \textbf{1.0} & \textbf{1.0} & 1.6\\
quadrotor\_0/empty\_1\_easy & 1.7 & 1.3 & \textbf{2.7} & - & - & - & \textbf{1.2} & \textbf{1.2} & 4.3\\
quadrotor\_0/window & \textbf{2.2} & \textbf{2.0} & 13.6 & - & - & - & 3.7 & 3.0 & \textbf{11.6}\\
quadrotor\_0/recovery & \textbf{2.5} & \textbf{2.4} & \textbf{9.4} & - & - & - & - & - & -\\
quadrotor\_0/recovery\_with\_obs & \textbf{4.1} & \textbf{3.2} & \textbf{9.4} & - & - & - & - & - & -\\
quadrotor\_0/quad\_one\_obs & \textbf{3.3} & \textbf{2.8} & 27.0 & - & - & - & 4.2 & 3.6 & \textbf{18.2}\\
quadrotor\_ompl/empty\_0\_easy & \textbf{0.8} & 0.8 & 0.3 & 0.9 & \textbf{0.8} & \textbf{0.2} & 1.0 & 1.0 & 0.6\\
quadrotor\_ompl/empty\_1\_easy & 0.9 & 0.9 & \textbf{0.5} & 2.6 & 3.3 & 4.6 & \textbf{0.9} & \textbf{0.9} & 1.4\\
quadrotor\_ompl/window & \textbf{3.5} & \textbf{2.4} & \textbf{3.6} & - & - & - & 4.2 & 3.2 & 10.7\\
quadrotor\_ompl/recovery & 2.1 & \textbf{1.9} & \textbf{5.5} & - & - & - & \textbf{2.0} & 2.0 & 22.6\\
quadrotor\_ompl/quad\_one\_obs & \textbf{2.7} & \textbf{2.2} & \textbf{3.4} & - & - & - & 2.7 & 3.0 & 11.5\\
quadrotor\_ompl/recovery\_with\_obs & \textbf{2.8} & \textbf{2.5} & \textbf{49.4} & - & - & - & - & - & -\\
\bottomrule
\end{tabular}


==> results_tmp/merged_2023-06-21--14-29-12.tex.nice.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
&  \multicolumn{3}{c}{idba*} & \multicolumn{3}{c}{sst*} & \multicolumn{3}{c}{geo}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& cf & cl & tf & cf & cl & tf & cf & cl & tf \\
\midrule
acrobot/swing\_up\_empty & 7.9 & 8.2 & \textbf{7.1} & - & - & - & \textbf{3.8} & \textbf{3.6} & 7.6\\
acrobot/swing\_up\_obs\_hard & 5.2 & 4.9 & 9.5 & - & - & - & \textbf{4.3} & \textbf{3.6} & \textbf{4.8}\\
car\_first\_order\_with\_1\_trailers\_0/kink\_0 & \textbf{24.2} & \textbf{15.1} & \textbf{2.6} & 56.2 & 66.0 & 5.7 & 27.3 & 22.3 & 20.3\\
quad2d/quad2d\_recovery\_obs & \textbf{4.5} & \textbf{4.5} & \textbf{11.6} & - & - & - & - & - & -\\
quad2d/quad\_bugtrap & \textbf{5.2} & \textbf{5.2} & \textbf{7.9} & - & - & - & - & - & -\\
quad2dpole/up\_obs & \textbf{4.0} & \textbf{3.9} & \textbf{4.8} & - & - & - & - & - & -\\
quad2dpole/window\_hard & \textbf{4.5} & \textbf{4.5} & \textbf{8.0} & - & - & - & - & - & -\\
quadrotor\_0/recovery & \textbf{2.5} & \textbf{2.4} & \textbf{9.4} & - & - & - & - & - & -\\
quadrotor\_0/recovery\_with\_obs & \textbf{4.1} & \textbf{3.2} & \textbf{9.4} & - & - & - & - & - & -\\
quadrotor\_ompl/window & \textbf{3.5} & \textbf{2.4} & \textbf{3.6} & - & - & - & 4.2 & 3.2 & 10.7\\
uni1\_0/bugtrap\_0 & \textbf{21.9} & \textbf{20.7} & 2.0 & 74.3 & 31.9 & \textbf{1.0} & 31.1 & 23.8 & 5.5\\
uni1\_0/kink\_0 & \textbf{21.5} & \textbf{13.2} & 1.5 & 49.1 & 19.3 & \textbf{0.5} & 24.7 & 13.8 & 2.7\\
uni1\_2/wall\_0 & \textbf{20.0} & \textbf{18.1} & \textbf{1.5} & 45.0 & 28.9 & 4.1 & - & - & -\\
uni2\_0/bugtrap\_0 & \textbf{26.2} & \textbf{25.1} & \textbf{1.9} & 66.2 & 61.1 & 6.3 & 32.2 & 31.4 & 38.1\\
uni2\_0/park & \textbf{5.8} & \textbf{5.8} & \textbf{0.3} & 22.4 & 10.0 & 0.6 & 5.9 & 5.8 & 0.7\\
\bottomrule
\end{tabular}


==> results_tmp/merged_2023-07-06--17-08-02.tex.nice.tex <==
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{idba*} & \multicolumn{4}{c}{sst} & \multicolumn{4}{c}{geo}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
 id & dyn & scene &  p & tf & cf & cl &  p & tf & cf & cl &  p & tf&  cf & cl  \\
\midrule
\#0 & car\_first\_order\_with\_1\_trailers\_0 & bugtrap\_0 & \textbf{1.0} & 1.7 & \textbf{22.4} & \textbf{19.0} & \textbf{1.0} & \textbf{0.4} & 60.1 & 42.9 & 0.3 & - & - & -\\
\#1 & car\_first\_order\_with\_1\_trailers\_0 & kink\_0 & \textbf{1.0} & 3.0 & \textbf{24.2} & \textbf{14.9} & \textbf{1.0} & \textbf{0.4} & 61.5 & 53.0 & \textbf{1.0} & 22.3 & 48.0 & 18.5\\
\#2 & car\_first\_order\_with\_1\_trailers\_0 & park & \textbf{1.0} & \textbf{1.4} & 8.7 & \textbf{4.4} & 0.4 & - & - & - & 0.7 & 2.2 & \textbf{7.6} & 5.8\\
\#3 & uni1\_0 & bugtrap\_0 & \textbf{1.0} & 2.2 & \textbf{21.9} & \textbf{20.7} & \textbf{1.0} & \textbf{0.2} & 69.4 & 24.4 & \textbf{1.0} & 11.4 & 45.5 & 24.4\\
\#4 & uni1\_0 & kink\_0 & \textbf{1.0} & 1.7 & \textbf{21.5} & \textbf{13.2} & \textbf{1.0} & \textbf{0.1} & 50.5 & 15.8 & \textbf{1.0} & 2.0 & 26.4 & 13.5\\
\#5 & uni1\_0 & park & \textbf{1.0} & 0.2 & 3.7 & \textbf{3.1} & \textbf{1.0} & \textbf{0.1} & 8.4 & 3.2 & \textbf{1.0} & \textbf{0.1} & \textbf{3.5} & \textbf{3.1}\\
\#6 & uni1\_1 & kink\_0 & \textbf{1.0} & \textbf{1.7} & \textbf{21.3} & \textbf{21.1} & \textbf{1.0} & 12.2 & 42.9 & 24.6 & \textbf{1.0} & 8.6 & 45.3 & 23.3\\
\#7 & uni1\_2 & wall\_0 & \textbf{1.0} & 1.5 & \textbf{19.5} & \textbf{18.0} & \textbf{1.0} & \textbf{0.4} & 48.0 & 21.5 & 0.1 & - & - & -\\
\#8 & uni2\_0 & bugtrap\_0 & \textbf{1.0} & 2.1 & \textbf{25.6} & \textbf{25.1} & \textbf{1.0} & \textbf{0.9} & 90.6 & 46.0 & \textbf{1.0} & 6.0 & 46.1 & 28.7\\
\#9 & uni2\_0 & kink\_0 & \textbf{1.0} & 1.3 & \textbf{17.8} & \textbf{17.7} & \textbf{1.0} & \textbf{1.0} & 83.0 & 40.2 & \textbf{1.0} & 3.0 & 33.2 & 18.0\\
\#10 & uni2\_0 & park & \textbf{1.0} & 0.3 & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.1} & 35.2 & 6.0 & \textbf{1.0} & 0.3 & 6.8 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp/merged_2023-07-12--19-29-01.tex.nice.tex <==
\begin{tabular}{cccrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{iDbA*} & \multicolumn{4}{c}{SST*} & \multicolumn{4}{c}{RRT*+TO}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
$ \# $ & Dynamics & Instance & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$\\
\midrule
0 & Acrobot & swing down & \textbf{1.0} & 5.3 & 5.3 & 5.3 & 0.0 & - & - & - & \textbf{1.0} & \textbf{1.9} & \textbf{4.0} & \textbf{3.2}\\
1 & Acrobot & swing down & \textbf{1.0} & \textbf{3.1} & \textbf{3.6} & \textbf{2.9} & 0.0 & - & - & - & 0.0 & - & - & -\\
2 & Acrobot & swing up & \textbf{1.0} & 6.0 & 6.9 & 5.0 & 0.4 & - & - & - & 0.8 & \textbf{1.5} & \textbf{4.0} & \textbf{4.0}\\
3 & Acrobot & swing up obstacles v0 & \textbf{1.0} & 6.6 & 6.3 & 5.0 & 0.4 & - & - & - & 0.7 & \textbf{4.2} & \textbf{6.0} & \textbf{3.9}\\
4 & Acrobot & swing up obstacles v1 & \textbf{1.0} & 7.2 & \textbf{6.2} & 5.0 & 0.1 & - & - & - & \textbf{1.0} & \textbf{5.3} & 6.6 & \textbf{3.4}\\
5 & Trailer & bugtrap & \textbf{1.0} & 1.8 & \textbf{22.3} & \textbf{19.0} & \textbf{1.0} & \textbf{0.7} & 55.3 & 44.6 & 0.3 & - & - & -\\
6 & Trailer & kink & \textbf{1.0} & 2.7 & \textbf{24.2} & \textbf{14.9} & \textbf{1.0} & \textbf{0.4} & 67.6 & 61.5 & \textbf{1.0} & 25.8 & 37.2 & 18.9\\
7 & Trailer & park & \textbf{1.0} & 1.6 & \textbf{8.7} & \textbf{4.1} & 0.9 & \textbf{0.5} & 12.0 & 9.8 & 0.6 & 3.2 & 9.9 & 5.8\\
8 & Planar Rotor & empty v0 & \textbf{1.0} & \textbf{0.1} & 1.0 & \textbf{1.0} & \textbf{1.0} & 0.3 & 1.8 & 1.1 & \textbf{1.0} & 0.2 & \textbf{1.0} & \textbf{1.0}\\
9 & Planar Rotor & empty v1 & \textbf{1.0} & 0.4 & 1.4 & \textbf{1.3} & \textbf{1.0} & 0.8 & 4.1 & 1.5 & \textbf{1.0} & \textbf{0.2} & \textbf{1.4} & 1.4\\
10 & Planar Rotor & holle & \textbf{0.9} & 41.6 & \textbf{3.4} & \textbf{3.0} & 0.7 & 77.6 & 12.4 & 8.4 & \textbf{0.9} & \textbf{40.0} & 4.1 & 3.3\\
11 & Planar Rotor & recovery obstacles & \textbf{1.0} & \textbf{13.7} & \textbf{4.6} & \textbf{4.4} & 0.0 & - & - & - & 0.5 & 91.4 & 4.8 & 4.8\\
12 & Planar Rotor & recovery & \textbf{1.0} & \textbf{0.5} & \textbf{3.1} & \textbf{3.1} & 0.0 & - & - & - & 0.0 & - & - & -\\
13 & Planar Rotor & bugtrap & \textbf{1.0} & \textbf{27.1} & \textbf{5.2} & \textbf{5.2} & \textbf{1.0} & 31.0 & 11.2 & 8.6 & \textbf{1.0} & 31.1 & 15.8 & 10.3\\
14 & Planar Rotor & column & \textbf{1.0} & 3.5 & \textbf{3.3} & \textbf{3.3} & \textbf{1.0} & 27.1 & 9.0 & 7.1 & \textbf{1.0} & \textbf{1.2} & 5.4 & 3.6\\
15 & Rotor Pole & down & \textbf{1.0} & \textbf{1.7} & \textbf{3.9} & \textbf{3.2} & 0.0 & - & - & - & \textbf{1.0} & 8.5 & 5.7 & 5.7\\
16 & Rotor Pole & move v1 & \textbf{1.0} & \textbf{0.4} & 2.4 & 2.4 & 0.3 & - & - & - & \textbf{1.0} & 1.6 & \textbf{2.4} & \textbf{2.4}\\
17 & Rotor Pole & move v0 & \textbf{1.0} & 1.9 & 5.2 & 3.9 & 0.0 & - & - & - & \textbf{1.0} & \textbf{1.6} & \textbf{3.1} & \textbf{3.1}\\
18 & Rotor Pole & up & \textbf{1.0} & 8.4 & \textbf{3.2} & \textbf{3.1} & 0.0 & - & - & - & \textbf{1.0} & \textbf{3.6} & 3.7 & 3.7\\
19 & Rotor Pole & swing up obstacles & \textbf{1.0} & \textbf{6.5} & \textbf{4.0} & \textbf{3.9} & 0.0 & - & - & - & 0.9 & 76.7 & 21.8 & 4.1\\
20 & Rotor Pole & window & \textbf{1.0} & \textbf{18.0} & \textbf{4.4} & \textbf{4.3} & 0.0 & - & - & - & 0.6 & 114.4 & 6.0 & 6.0\\
21 & Rotor Pole & column & \textbf{1.0} & \textbf{27.2} & \textbf{4.1} & \textbf{3.2} & 0.0 & - & - & - & 0.4 & - & - & -\\
22 & Rotor Pole & small window & \textbf{1.0} & \textbf{10.0} & \textbf{4.5} & \textbf{4.5} & 0.0 & - & - & - & 0.2 & - & - & -\\
23 & Quadcopter Force & empty v0 & \textbf{1.0} & 0.4 & 1.4 & 1.4 & 0.0 & - & - & - & \textbf{1.0} & \textbf{0.2} & \textbf{1.0} & \textbf{1.0}\\
24 & Quadcopter Force & empty v1 & \textbf{1.0} & 1.2 & 2.5 & 1.4 & 0.0 & - & - & - & \textbf{1.0} & \textbf{0.4} & \textbf{1.2} & \textbf{1.2}\\
25 & Quadcopter Force & obstacle & \textbf{1.0} & 4.3 & 6.2 & \textbf{3.1} & 0.0 & - & - & - & \textbf{1.0} & \textbf{2.7} & \textbf{5.7} & 3.5\\
26 & Quadcopter Force & recovery & \textbf{1.0} & \textbf{2.0} & \textbf{6.1} & \textbf{2.4} & 0.0 & - & - & - & 0.0 & - & - & -\\
27 & Quadcopter Force & recovery obstacles & \textbf{1.0} & \textbf{3.1} & 5.7 & 3.6 & 0.0 & - & - & - & \textbf{1.0} & \textbf{3.1} & \textbf{5.5} & \textbf{3.1}\\
28 & Quadcopter Force & window & \textbf{1.0} & 6.8 & 4.4 & \textbf{2.4} & 0.0 & - & - & - & \textbf{1.0} & \textbf{2.0} & \textbf{3.7} & 2.6\\
29 & Quadcopter Thrust & empty v0 & \textbf{1.0} & 0.3 & 0.9 & 0.9 & 0.8 & \textbf{0.1} & \textbf{0.9} & \textbf{0.9} & \textbf{1.0} & 0.2 & 1.0 & 1.0\\
30 & Quadcopter Thrust & empty v1 & \textbf{1.0} & 0.4 & 1.6 & 1.2 & 0.9 & 4.2 & 5.2 & 3.0 & \textbf{1.0} & \textbf{0.2} & \textbf{0.9} & \textbf{0.9}\\
31 & Quadcopter Thrust & obstacle & \textbf{1.0} & 3.5 & \textbf{2.9} & \textbf{2.7} & 0.1 & - & - & - & \textbf{1.0} & \textbf{2.3} & 4.8 & 3.6\\
32 & Quadcopter Thrust & recovery & \textbf{1.0} & \textbf{0.6} & 2.2 & 2.1 & 0.0 & - & - & - & 0.8 & 1.4 & \textbf{2.0} & \textbf{2.0}\\
33 & Quadcopter Thrust & recovery obstacles & \textbf{1.0} & \textbf{2.6} & \textbf{3.1} & 3.0 & 0.0 & - & - & - & \textbf{1.0} & 3.0 & 5.0 & \textbf{2.6}\\
34 & Quadcopter Thrust & window & \textbf{1.0} & \textbf{1.9} & \textbf{2.5} & \textbf{2.2} & 0.4 & - & - & - & \textbf{1.0} & 2.3 & 5.7 & 2.5\\
35 & Unicycle 1 v0 & bugtrap & \textbf{1.0} & 2.2 & \textbf{22.0} & \textbf{20.7} & \textbf{1.0} & \textbf{0.2} & 72.8 & 24.0 & \textbf{1.0} & 3.3 & 38.2 & 23.4\\
36 & Unicycle 1 v0 & kink & \textbf{1.0} & 1.7 & \textbf{21.5} & \textbf{13.2} & \textbf{1.0} & \textbf{0.1} & 73.8 & 15.2 & \textbf{1.0} & 2.0 & 24.5 & 14.1\\
37 & Unicycle 1 v0 & park & \textbf{1.0} & 0.3 & 3.7 & \textbf{3.1} & \textbf{1.0} & \textbf{0.1} & 8.9 & \textbf{3.1} & \textbf{1.0} & \textbf{0.1} & \textbf{3.4} & \textbf{3.1}\\
38 & Unicycle 1 v1 & kink & \textbf{1.0} & \textbf{1.7} & \textbf{21.4} & \textbf{21.1} & \textbf{1.0} & 11.2 & 45.7 & 24.3 & \textbf{1.0} & 4.6 & 41.3 & 23.2\\
39 & Unicycle 1 v2 & wall & \textbf{1.0} & 1.6 & \textbf{19.8} & \textbf{18.0} & \textbf{1.0} & \textbf{0.4} & 46.6 & 20.5 & 0.3 & - & - & -\\
40 & Unicycle 2 & bugtrap & \textbf{1.0} & 2.3 & \textbf{25.9} & \textbf{25.1} & \textbf{1.0} & \textbf{0.7} & 75.1 & 46.7 & \textbf{1.0} & 7.0 & 54.8 & 29.0\\
41 & Unicycle 2 & kink & \textbf{1.0} & 1.3 & \textbf{17.7} & \textbf{17.7} & \textbf{1.0} & \textbf{0.8} & 73.1 & 38.1 & \textbf{1.0} & 3.3 & 31.5 & 20.4\\
42 & Unicycle 2 & park & \textbf{1.0} & 0.3 & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.2} & 24.6 & 5.9 & \textbf{1.0} & 0.3 & 6.6 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp/merged_2023-07-17--17-12-03.tex.nice.tex <==
\begin{tabular}{cccrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{iDbA*} & \multicolumn{4}{c}{SST*} & \multicolumn{4}{c}{RRT*+TO}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
 \# & System & Instance & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$\\
\midrule
0 & Acrobot & swing up & \textbf{1.0} & 6.0 & 6.9 & 5.0 & 0.4 & - & - & - & 0.8 & \textbf{1.5} & \textbf{4.0} & \textbf{4.0}\\
1 & Acrobot & swing up obstacles v1 & \textbf{1.0} & 7.2 & \textbf{6.2} & 5.0 & 0.1 & - & - & - & \textbf{1.0} & \textbf{5.3} & 6.6 & \textbf{3.4}\\
2 & Trailer & kink & \textbf{1.0} & 2.7 & \textbf{24.2} & \textbf{14.9} & \textbf{1.0} & \textbf{0.4} & 67.6 & 61.5 & \textbf{1.0} & 25.8 & 37.2 & 18.9\\
3 & Trailer & park & \textbf{1.0} & 1.6 & \textbf{8.7} & \textbf{4.1} & 0.9 & \textbf{0.5} & 12.0 & 9.8 & 0.6 & 3.2 & 9.9 & 5.8\\
4 & Planar Rotor & hole & \textbf{0.9} & 41.6 & \textbf{3.4} & \textbf{3.0} & 0.7 & 77.6 & 12.4 & 8.4 & \textbf{0.9} & \textbf{40.0} & 4.1 & 3.3\\
5 & Planar Rotor & bugtrap & \textbf{1.0} & \textbf{27.1} & \textbf{5.2} & \textbf{5.2} & \textbf{1.0} & 31.0 & 11.2 & 8.6 & \textbf{1.0} & 31.1 & 15.8 & 10.3\\
6 & Rotor Pole & swing up obstacles & \textbf{1.0} & \textbf{6.5} & \textbf{4.0} & \textbf{3.9} & 0.0 & - & - & - & 0.9 & 76.7 & 21.8 & 4.1\\
7 & Rotor Pole & small window & \textbf{1.0} & \textbf{10.0} & \textbf{4.5} & \textbf{4.5} & 0.0 & - & - & - & 0.2 & - & - & -\\
8 & Quadcopter Force & recovery & \textbf{1.0} & \textbf{2.0} & \textbf{6.1} & \textbf{2.4} & 0.0 & - & - & - & 0.0 & - & - & -\\
9 & Quadcopter Force & recovery obstacles & \textbf{1.0} & \textbf{3.1} & 5.7 & 3.6 & 0.0 & - & - & - & \textbf{1.0} & \textbf{3.1} & \textbf{5.5} & \textbf{3.1}\\
10 & Quadcopter Thrust & obstacle & \textbf{1.0} & 3.5 & \textbf{2.9} & \textbf{2.7} & 0.1 & - & - & - & \textbf{1.0} & \textbf{2.3} & 4.8 & 3.6\\
11 & Quadcopter Thrust & window & \textbf{1.0} & \textbf{1.9} & \textbf{2.5} & \textbf{2.2} & 0.4 & - & - & - & \textbf{1.0} & 2.3 & 5.7 & 2.5\\
12 & Unicycle 1 v0 & bugtrap & \textbf{1.0} & 2.2 & \textbf{22.0} & \textbf{20.7} & \textbf{1.0} & \textbf{0.2} & 72.8 & 24.0 & \textbf{1.0} & 3.3 & 38.2 & 23.4\\
13 & Unicycle 1 v2 & wall & \textbf{1.0} & 1.6 & \textbf{19.8} & \textbf{18.0} & \textbf{1.0} & \textbf{0.4} & 46.6 & 20.5 & 0.3 & - & - & -\\
14 & Unicycle 2 & bugtrap & \textbf{1.0} & 2.3 & \textbf{25.9} & \textbf{25.1} & \textbf{1.0} & \textbf{0.7} & 75.1 & 46.7 & \textbf{1.0} & 7.0 & 54.8 & 29.0\\
15 & Unicycle 2 & park & \textbf{1.0} & 0.3 & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.2} & 24.6 & 5.9 & \textbf{1.0} & 0.3 & 6.6 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp/summary_search_2023-06-06--13-53-25.tex <==
\begin{tabular}{ccccccc}
\toprule
&   \multicolumn{2}{c}{eucl} & \multicolumn{2}{c}{roadmap} & \multicolumn{2}{c}{blind} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
&   n & t & n & t & n & t  \\
\midrule
uni1\_0/park & 21.0 & \textbf{2.3} & \textbf{20.0} & 4.6 & 126.0 & 10.7\\
uni1\_0/bugtrap\_0 & 20038.0 & 2261.2 & \textbf{6801.0} & \textbf{1127.8} & 28033.0 & 3108.0\\
uni1\_0/kink\_0 & 3540.0 & \textbf{369.6} & \textbf{2910.0} & 391.8 & 10527.0 & 1056.7\\
uni2\_0/kink\_0 & 19416.2 & 2207.5 & \textbf{3070.2} & \textbf{364.3} & 33117.0 & 3909.2\\
uni2\_0/park & \textbf{38.0} & \textbf{3.2} & 88.0 & 13.1 & 182.5 & 14.2\\
uni2\_0/bugtrap\_0 & 75080.8 & 9197.4 & \textbf{53425.2} & \textbf{8273.1} & 84648.5 & 9986.0\\
\bottomrule
\end{tabular}


==> results_tmp/summary_search_2023-06-22--20-41-46.tex <==
\begin{tabular}{lcccccc}
\toprule
&   \multicolumn{2}{c}{eucl} & \multicolumn{2}{c}{roadmap} & \multicolumn{2}{c}{blind} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
&   n & t & n & t & n & t  \\
\midrule
quad2d/quad\_bugtrap & 39694.0 & 6712.9 & \textbf{17601.0} & \textbf{3354.0} & 80959.0 & 13839.2\\
quadrotor\_0/quad\_one\_obs & 70706.0 & 30928.7 & \textbf{36256.0} & \textbf{24642.9} & 131972.0 & 60001.6\\
uni1\_0/bugtrap\_0 & 19722.0 & 2937.5 & \textbf{4923.0} & \textbf{991.0} & 28319.0 & 3819.0\\
uni2\_0/bugtrap\_0 & 75708.0 & 12452.8 & \textbf{44009.0} & \textbf{9055.8} & 87013.0 & 13905.2\\
\bottomrule
\end{tabular}


==> results_tmp/summary_search_2023-06-22--21-00-08.tex <==
\begin{tabular}{lcccccc}
\toprule
&   \multicolumn{2}{c}{eucl} & \multicolumn{2}{c}{roadmap} & \multicolumn{2}{c}{blind} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
&   n & t & n & t & n & t  \\
\midrule
quad2d/quad\_bugtrap & 39694.0 & 6712.9 & \textbf{17601.0} & \textbf{3354.0} & 80959.0 & 13839.2\\
quadrotor\_0/quad\_one\_obs & 70706.0 & 30928.7 & \textbf{36256.0} & \textbf{24642.9} & - & -\\
uni1\_0/bugtrap\_0 & 19722.0 & 2937.5 & \textbf{4923.0} & \textbf{991.0} & 28319.0 & 3819.0\\
uni2\_0/bugtrap\_0 & 75708.0 & 12452.8 & \textbf{44009.0} & \textbf{9055.8} & 87013.0 & 13905.2\\
\bottomrule
\end{tabular}


==> results_tmp/summary_search_2023-07-06--19-54-37.tex <==
\begin{tabular}{llcccccc}
\toprule
 & &   \multicolumn{2}{c}{eucl} & \multicolumn{2}{c}{roadmap} & \multicolumn{2}{c}{blind} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 dynamics & scene & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t[s]  \\
\midrule
car\_first\_order\_with\_1\_trailers\_0 & bugtrap\_0 & 15.6 & 9.0 & \textbf{0.1} & \textbf{0.1} & 35.6 & 18.7\\
quad2d & quad\_bugtrap & 39.7 & 5.4 & \textbf{17.7} & \textbf{2.7} & 81.1 & 10.9\\
quad2dpole & window & 44.8 & \textbf{12.0} & \textbf{31.9} & 13.1 & 78.7 & 20.1\\
quadrotor\_0 & quad\_one\_obs & 69.8 & 24.9 & \textbf{36.7} & \textbf{20.0} & - & -\\
quadrotor\_0 & window & 8.0 & \textbf{1.5} & \textbf{7.0} & 8.0 & 32.4 & 11.4\\
uni1\_0 & bugtrap\_0 & 19.7 & 2.1 & \textbf{4.9} & \textbf{0.8} & 28.3 & 2.8\\
uni2\_0 & bugtrap\_0 & 75.7 & 9.6 & \textbf{44.0} & \textbf{6.9} & 87.0 & 10.8\\
\bottomrule
\end{tabular}


==> results_tmp/summary_search_2023-07-13--19-07-27.tex <==
\begin{tabular}{llcccccc}
\toprule
 & &   \multicolumn{2}{c}{Euclidean} & \multicolumn{2}{c}{Roadmap} & \multicolumn{2}{c}{Blind} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 Dynamics & Instance & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t [s]\\
\midrule
Trailer & bugtrap & 11.6 & 0.5 & \textbf{4.5} & \textbf{0.1} & 24.1 & 0.7\\
Planar Rotor & bugtrap & 117.3 & 15.0 & \textbf{45.3} & \textbf{6.1} & 229.7 & 30.0\\
Rotor Pole & window & 44.9 & \textbf{9.3} & \textbf{31.9} & 10.2 & 78.8 & 17.5\\
Quadcopter Force & obstacle & 71.0 & 20.0 & \textbf{38.9} & \textbf{15.7} & 169.8 & 60.0\\
Quadcopter Force & window & 8.5 & \textbf{1.8} & \textbf{6.9} & 5.9 & 33.4 & 9.1\\
Unicycle 1 v0 & bugtrap & 19.7 & 1.5 & \textbf{4.9} & \textbf{0.5} & 28.3 & 2.0\\
Unicycle 2 & bugtrap & 75.7 & 6.5 & \textbf{44.0} & \textbf{5.3} & 87.0 & 7.7\\
\bottomrule
\end{tabular}


==> results_tmp/summary_timeopt_2023-06-22--19-08-39.tex <==
\begin{tabular}{lcccccccc}
\toprule
&   \multicolumn{2}{c}{dt} & \multicolumn{2}{c}{search} & \multicolumn{2}{c}{mpc}
& \multicolumn{2}{c}{mpcc} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
&   c & t & c & t & c & t & c & t \\
\midrule
unicycle1\_v0/bugtrap\_0/delta\_02\_v0 & \textbf{20.9} & 1250.0 & 22.1 & 986.0 & 22.0 & \textbf{217.8} & 24.6 & 822.6\\
unicycle1\_v0/bugtrap\_0/delta\_05\_v0 & \textbf{21.1} & 1340.8 & 22.3 & 1135.9 & 24.0 & \textbf{162.9} & 21.4 & 774.3\\
unicycle2\_v0/bugtrap\_0/delta\_02\_v0 & \textbf{25.5} & 770.8 & 27.8 & 1147.7 & 36.0 & \textbf{348.2} & 58.2 & 2040.9\\
unicycle2\_v0/bugtrap\_0/delta\_05\_v0 & \textbf{25.1} & 537.5 & 26.3 & 1195.6 & 32.0 & \textbf{507.0} & 29.8 & 1095.2\\
quad2d/bugtrap/delta\_05\_v0 & 5.2 & 2184.0 & \textbf{4.8} & 9509.3 & 6.0 & \textbf{1323.3} & 5.0 & 3352.1\\
quad2d/bugtrap/delta\_045\_v0 & 5.0 & 3082.0 & \textbf{4.8} & 9166.3 & 5.4 & \textbf{1678.1} & 5.0 & 4630.7\\
\bottomrule
\end{tabular}


==> results_tmp/summary_timeopt_2023-07-07--15-59-23.tex <==
\begin{tabular}{lllcccccccc}
\toprule
 & & &   \multicolumn{2}{c}{dt} & \multicolumn{2}{c}{search} & \multicolumn{2}{c}{mpc}
& \multicolumn{2}{c}{mpcc} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
& & &   c [s] & t [ms] & c [s] & t [ms] & c [s] & t [ms] & c [s] & t [ms] \\
\midrule
quad2d & bugtrap & delta\_045\_v0 & 5.0 & \textbf{4033.9} & \textbf{4.8} & 14005.7 & \textbf{-} & \textbf{-} & 5.0 & 5877.5\\
quad2d & bugtrap & delta\_04\_v0 & \textbf{5.4} & 6393.3 & 5.8 & 12378.0 & 6.8 & \textbf{3810.6} & 6.0 & 7291.8\\
quad2d & bugtrap & delta\_05\_v0 & 5.2 & 2697.5 & \textbf{4.8} & 12371.3 & 6.0 & \textbf{1555.3} & 5.0 & 4138.4\\
quad2d & bugtrap & delta\_10\_v0 & \textbf{4.3} & \textbf{4362.2} & 4.7 & 14319.6 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & bugtrap & delta\_15\_v0 & 4.9 & \textbf{3687.5} & \textbf{4.2} & 13316.7 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & bugtrap & delta\_20\_v0 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & recovery\_wo\_obs & delta\_03\_v0 & \textbf{3.3} & 4503.7 & 3.6 & 6839.2 & \textbf{-} & \textbf{-} & 4.0 & \textbf{1253.9}\\
quad2d & recovery\_wo\_obs & delta\_04\_v0 & \textbf{3.2} & 4668.9 & 3.5 & 6256.7 & \textbf{-} & \textbf{-} & 4.0 & \textbf{1521.9}\\
quad2d & recovery\_wo\_obs & delta\_05\_v0 & 3.2 & \textbf{4559.9} & \textbf{2.7} & 8358.5 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & recovery\_wo\_obs & delta\_08\_v0 & \textbf{3.1} & \textbf{5012.5} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & recovery\_wo\_obs & delta\_10\_v0 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quad2d & recovery\_wo\_obs & delta\_15\_v0 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_05\_v0 & 5.5 & 3738.0 & \textbf{2.7} & 6422.5 & 5.8 & \textbf{2722.3} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_06\_v0 & 5.6 & 6489.6 & \textbf{2.9} & 7052.3 & 5.8 & \textbf{3809.2} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_07\_v0 & 6.8 & 7102.0 & \textbf{2.5} & 5798.0 & 5.4 & \textbf{2917.8} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_08\_v0 & 4.2 & 5674.3 & \textbf{2.5} & 7123.2 & 3.8 & \textbf{2986.2} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_10\_v0 & 2.9 & 4705.9 & \textbf{2.4} & 8436.3 & 3.4 & \textbf{1964.3} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & recovery & delta\_15\_v0 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & window & window\_05\_v0 & \textbf{3.4} & 6455.1 & 3.5 & 8648.5 & 4.2 & \textbf{2780.3} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & window & window\_06\_v0 & 5.2 & 8717.8 & \textbf{3.7} & 9089.3 & 7.0 & \textbf{4911.7} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & window & window\_08\_v0 & \textbf{3.2} & 3866.0 & 3.4 & 11991.9 & 3.8 & \textbf{3030.4} & \textbf{-} & \textbf{-}\\
quadrotor\_0 & window & window\_15\_v0 & 3.4 & 4847.8 & \textbf{3.2} & 16721.8 & 3.8 & \textbf{3719.0} & \textbf{-} & \textbf{-}\\
unicycle1\_v0 & bugtrap\_0 & delta\_02\_v0 & \textbf{20.9} & 1490.9 & 22.1 & 1258.0 & 22.0 & \textbf{310.5} & 22.8 & 1071.1\\
unicycle1\_v0 & bugtrap\_0 & delta\_03\_v0 & \textbf{20.8} & 2038.1 & 21.8 & 1151.6 & 26.0 & \textbf{248.1} & 23.2 & 1140.2\\
unicycle1\_v0 & bugtrap\_0 & delta\_05\_v0 & \textbf{21.1} & 1522.0 & 22.3 & 1411.3 & 24.0 & \textbf{222.9} & 21.4 & 1094.5\\
unicycle1\_v0 & bugtrap\_0 & delta\_10\_v0 & \textbf{24.8} & 1963.9 & 29.4 & 1623.5 & 32.0 & \textbf{374.8} & 25.6 & 1184.9\\
unicycle1\_v0 & bugtrap\_0 & delta\_13\_v1 & 35.2 & 2009.4 & 31.4 & 1968.3 & 38.0 & \textbf{424.6} & \textbf{29.8} & 1446.3\\
unicycle2\_v0 & bugtrap\_0 & delta\_02\_v0 & \textbf{25.8} & 931.5 & 27.8 & 1518.4 & 36.0 & \textbf{601.2} & 40.9 & 2056.9\\
unicycle2\_v0 & bugtrap\_0 & delta\_03\_v0 & 25.4 & 981.8 & \textbf{25.1} & 1372.0 & 32.0 & \textbf{682.0} & 29.0 & 1348.3\\
unicycle2\_v0 & bugtrap\_0 & delta\_05\_v0 & \textbf{25.1} & 726.3 & 26.3 & 1645.6 & 32.0 & \textbf{647.9} & \textbf{-} & \textbf{-}\\
unicycle2\_v0 & bugtrap\_0 & delta\_10\_v0 & \textbf{25.1} & \textbf{728.8} & 27.6 & 1834.9 & 32.0 & 832.9 & 29.2 & 1421.1\\
unicycle2\_v0 & bugtrap\_0 & delta\_15\_v0 & \textbf{25.2} & \textbf{885.0} & 27.8 & 1726.2 & 42.0 & 985.3 & 31.6 & 1526.4\\
\bottomrule
\end{tabular}


==> results_tmp/summary_timeopt_2023-07-12--20-50-29.tex <==
\begin{tabular}{llcccccccccc}
\toprule
 & & & &  \multicolumn{2}{c}{dt} & \multicolumn{2}{c}{search} & \multicolumn{2}{c}{mpc}
& \multicolumn{2}{c}{mpcc} \\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
System & Instance & $\delta$ & K  & J[s] & t[s] & J[s] & t[s] & J[s] & t[s] & J[s] & t[s] \\
\midrule
Planar Rotor & bugtrap & 0.4 & 614 & 5.4 & 0.7 & \textbf{4.2} & 1.0 & 6.2 & \textbf{0.3} & 4.6 & 1.5\\
Planar Rotor & bugtrap & 0.5 & 458 & 5.1 & 0.5 & 4.8 & 2.3 & 5.4 & \textbf{0.2} & \textbf{4.8} & 1.5\\
Planar Rotor & bugtrap & 1.0 & 373 & 4.7 & \textbf{0.4} & \textbf{4.7} & 2.1 & \textbf{-} & \textbf{-} & 6.3 & 1.8\\
Planar Rotor & bugtrap & 1.5 & 335 & 4.6 & \textbf{0.5} & \textbf{4.2} & 2.6 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
Planar Rotor & bugtrap & 2.0 & 365 & \textbf{5.3} & \textbf{0.6} & 5.5 & 3.4 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
Planar Rotor & recovery & 0.3 & 333 & \textbf{3.2} & 0.2 & 3.5 & 0.3 & 3.8 & \textbf{0.2} & 3.9 & 1.3\\
Planar Rotor & recovery & 0.4 & 329 & \textbf{3.2} & 0.2 & 3.5 & 0.3 & 3.8 & \textbf{0.2} & 3.4 & 1.4\\
Planar Rotor & recovery & 0.5 & 307 & \textbf{3.1} & \textbf{0.2} & 3.2 & 0.3 & \textbf{-} & \textbf{-} & 3.4 & 1.2\\
Planar Rotor & recovery & 0.8 & 237 & 3.0 & \textbf{0.3} & \textbf{3.0} & 0.3 & \textbf{-} & \textbf{-} & 3.8 & 2.0\\
Planar Rotor & recovery & 1.0 & 219 & \textbf{3.0} & \textbf{0.2} & 3.1 & 0.4 & \textbf{-} & \textbf{-} & 3.3 & 1.5\\
Planar Rotor & recovery & 1.5 & 56 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}\\
Quadcopter Force & recovery & 0.5 & 422 & 3.5 & \textbf{0.6} & \textbf{2.9} & 0.9 & 4.2 & 1.2 & 4.6 & 2.0\\
Quadcopter Force & recovery & 0.6 & 451 & 3.7 & 0.9 & \textbf{2.2} & \textbf{0.6} & 5.0 & 2.8 & 5.2 & 2.0\\
Quadcopter Force & recovery & 0.7 & 395 & 3.2 & \textbf{0.7} & \textbf{2.7} & 0.8 & 4.2 & 2.0 & \textbf{-} & \textbf{-}\\
Quadcopter Force & recovery & 0.8 & 236 & \textbf{2.4} & \textbf{0.4} & 2.5 & 1.3 & 2.6 & 1.2 & \textbf{-} & \textbf{-}\\
Quadcopter Force & recovery & 1.0 & 170 & 2.2 & \textbf{0.3} & \textbf{2.1} & 0.6 & 2.6 & 1.7 & \textbf{-} & \textbf{-}\\
Quadcopter Force & recovery & 1.5 & 40 & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{2.2} & \textbf{1.1} & \textbf{-} & \textbf{-}\\
Quadcopter Force & window & 0.5 & 425 & 3.4 & 1.7 & \textbf{2.9} & 1.9 & 4.2 & 2.0 & 4.4 & \textbf{0.9}\\
Quadcopter Force & window & 0.6 & 658 & 5.2 & 2.0 & \textbf{3.2} & 2.7 & 7.0 & 4.0 & 6.5 & \textbf{1.8}\\
Quadcopter Force & window & 0.8 & 318 & 2.8 & \textbf{1.0} & \textbf{2.8} & 1.9 & 3.8 & 2.0 & 4.6 & 1.2\\
Quadcopter Force & window & 1.5 & 311 & 2.9 & \textbf{1.2} & \textbf{2.8} & 3.0 & 3.8 & 3.0 & \textbf{-} & \textbf{-}\\
unicycle1\_v0 & bugtrap & 0.2 & 209 & \textbf{20.8} & 0.9 & 22.1 & 0.8 & 22.0 & \textbf{0.1} & 21.0 & 0.6\\
unicycle1\_v0 & bugtrap & 0.3 & 251 & \textbf{21.5} & 1.3 & 21.8 & 0.7 & 26.0 & \textbf{0.1} & 25.6 & 0.6\\
unicycle1\_v0 & bugtrap & 0.5 & 211 & 21.1 & 1.0 & 22.3 & 0.9 & 24.0 & \textbf{0.1} & \textbf{21.0} & 0.6\\
unicycle1\_v0 & bugtrap & 1.0 & 278 & \textbf{25.0} & 1.4 & 29.4 & 1.1 & 32.0 & \textbf{0.1} & 27.6 & 0.8\\
unicycle1\_v0 & bugtrap & 1.3 & 362 & 30.5 & 1.7 & 31.4 & 1.3 & 38.0 & \textbf{0.2} & \textbf{29.4} & 0.9\\
unicycle2\_v0 & bugtrap & 0.2 & 320 & \textbf{26.3} & 0.5 & 27.8 & 0.8 & 36.0 & \textbf{0.2} & 28.9 & 0.6\\
unicycle2\_v0 & bugtrap & 0.3 & 289 & 25.2 & 0.4 & \textbf{25.1} & 0.7 & 32.0 & \textbf{0.3} & 29.0 & 0.6\\
unicycle2\_v0 & bugtrap & 0.5 & 249 & \textbf{25.1} & 0.3 & 26.3 & 0.9 & 32.0 & \textbf{0.2} & 31.0 & 0.7\\
unicycle2\_v0 & bugtrap & 1.0 & 261 & \textbf{25.1} & 0.4 & 27.6 & 1.1 & 32.0 & \textbf{0.4} & 27.4 & 0.6\\
unicycle2\_v0 & bugtrap & 1.5 & 263 & \textbf{25.1} & \textbf{0.4} & 27.8 & 1.0 & 42.0 & 0.5 & 31.0 & 0.8\\
\bottomrule
\end{tabular}


==> results_tmp/summary_timeopt_2023-07-18--12-39-48.tex <==
\begin{tabular}{llcccccccccc}
\toprule
 & & & &  \multicolumn{2}{c}{dt} & \multicolumn{2}{c}{search} & \multicolumn{2}{c}{mpc}
& \multicolumn{2}{c}{mpcc} \\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
System & Instance & $\delta$ & K  & J[s] & t[s] & J[s] & t[s] & J[s] & t[s] & J[s] & t[s] \\
\midrule
Planar Rotor & bugtrap & 0.4 & 614 & 5.4 & 0.7 & \textbf{4.2} & 1.0 & 6.2 & \textbf{0.3} & 4.6 & 1.5\\
Planar Rotor & bugtrap & 1.0 & 373 & 4.7 & \textbf{0.4} & \textbf{4.7} & 2.1 & \textbf{-} & \textbf{-} & 6.3 & 1.8\\
Planar Rotor & recovery & 0.3 & 333 & \textbf{3.2} & 0.2 & 3.5 & 0.3 & 3.8 & \textbf{0.2} & 3.9 & 1.3\\
Planar Rotor & recovery & 0.8 & 237 & 3.0 & \textbf{0.3} & \textbf{3.0} & 0.3 & \textbf{-} & \textbf{-} & 3.8 & 2.0\\
Quadcopter Force & recovery & 0.5 & 422 & 3.5 & \textbf{0.6} & \textbf{2.9} & 0.9 & 4.2 & 1.2 & 4.6 & 2.0\\
Quadcopter Force & recovery & 1.0 & 170 & 2.2 & \textbf{0.3} & \textbf{2.1} & 0.6 & 2.6 & 1.7 & \textbf{-} & \textbf{-}\\
Quadcopter Force & window & 0.5 & 425 & 3.4 & 1.7 & \textbf{2.9} & 1.9 & 4.2 & 2.0 & 4.4 & \textbf{0.9}\\
Quadcopter Force & window & 0.8 & 318 & 2.8 & \textbf{1.0} & \textbf{2.8} & 1.9 & 3.8 & 2.0 & 4.6 & 1.2\\
unicycle1\_v0 & bugtrap & 0.2 & 209 & \textbf{20.8} & 0.9 & 22.1 & 0.8 & 22.0 & \textbf{0.1} & 21.0 & 0.6\\
unicycle2\_v0 & bugtrap & 1.0 & 261 & \textbf{25.1} & 0.4 & 27.6 & 1.1 & 32.0 & \textbf{0.4} & 27.4 & 0.6\\
\bottomrule
\end{tabular}


==> results_tmp/tmp_search.tex <==
\begin{tabular}{lllcccccccc}
\toprule
 & & &   \multicolumn{2}{c}{dt} & \multicolumn{2}{c}{search} & \multicolumn{2}{c}{mpc}
& \multicolumn{2}{c}{mpcc} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
& & &   c [s] & t [ms] & c [s] & t [ms] & c [s] & t [ms] & c [s] & t [ms] \\
\midrule
unicycle1\_v0 & bugtrap\_0 & delta\_03\_v0 & \textbf{20.8} & 1182.9 & 21.8 & 539.8 & 26.0 & \textbf{58.8} & 23.0 & 396.3\\
unicycle1\_v0 & bugtrap\_0 & delta\_02\_v0 & \textbf{20.9} & 779.4 & 22.1 & 619.6 & 22.0 & \textbf{110.7} & 23.0 & 449.7\\
unicycle1\_v0 & bugtrap\_0 & delta\_13\_v1 & 35.2 & 1141.3 & 31.4 & 999.9 & 38.0 & \textbf{140.0} & \textbf{29.7} & 647.5\\
unicycle1\_v0 & bugtrap\_0 & delta\_10\_v0 & \textbf{24.8} & 1132.3 & 29.4 & 863.9 & 32.0 & \textbf{115.8} & 26.2 & 536.6\\
unicycle1\_v0 & bugtrap\_0 & delta\_05\_v0 & \textbf{21.1} & 936.5 & 22.3 & 736.5 & 24.0 & \textbf{67.6} & 24.2 & 503.1\\
unicycle2\_v0 & bugtrap\_0 & delta\_02\_v0 & \textbf{26.0} & 408.5 & 27.8 & 626.3 & 36.0 & \textbf{143.4} & 28.9 & 587.3\\
unicycle2\_v0 & bugtrap\_0 & delta\_03\_v0 & 25.3 & 398.5 & \textbf{25.1} & 592.2 & 32.0 & \textbf{209.1} & 29.0 & 575.4\\
unicycle2\_v0 & bugtrap\_0 & delta\_05\_v0 & \textbf{25.1} & 336.7 & 26.3 & 766.1 & 32.0 & \textbf{199.5} & \textbf{-} & 699.5\\
unicycle2\_v0 & bugtrap\_0 & delta\_10\_v0 & \textbf{25.1} & 338.0 & 27.6 & 874.8 & 32.0 & \textbf{296.6} & \textbf{-} & 693.7\\
unicycle2\_v0 & bugtrap\_0 & delta\_15\_v0 & \textbf{25.2} & \textbf{390.3} & 27.8 & 818.8 & 42.0 & 393.1 & 31.6 & 754.6\\
quad2d & bugtrap & delta\_05\_v0 & 5.2 & 1467.8 & \textbf{4.8} & 7053.6 & 6.0 & \textbf{696.8} & 5.0 & 2146.9\\
quad2d & bugtrap & delta\_045\_v0 & 5.0 & 2028.4 & \textbf{4.8} & 8165.6 & \textbf{-} & \textbf{1075.0} & 5.0 & 3354.5\\
quad2d & bugtrap & delta\_04\_v0 & \textbf{5.4} & 3620.8 & 5.4 & 10069.4 & 6.8 & \textbf{2127.3} & 6.0 & 4383.3\\
quad2d & bugtrap & delta\_10\_v0 & \textbf{4.3} & 2754.0 & 4.7 & 8777.8 & \textbf{-} & \textbf{2075.0} & \textbf{-} & 2487.0\\
quad2d & bugtrap & delta\_20\_v0 & \textbf{-} & 2661.4 & \textbf{-} & 16557.0 & \textbf{-} & \textbf{1003.7} & \textbf{-} & 5528.4\\
quad2d & bugtrap & delta\_15\_v0 & 4.9 & 2248.4 & \textbf{4.2} & 7766.7 & \textbf{-} & \textbf{1184.7} & \textbf{-} & 4795.2\\
quadrotor\_0 & window & window\_05\_v0 & \textbf{3.4} & 7947.0 & 3.5 & 5545.7 & 4.2 & \textbf{1397.9} & \textbf{-} & 2090.3\\
quadrotor\_0 & window & window\_06\_v0 & 5.1 & 10988.2 & \textbf{4.1} & 6329.9 & 7.0 & \textbf{3019.2} & \textbf{-} & 3084.4\\
quadrotor\_0 & window & window\_15\_v0 & 3.3 & 5939.5 & \textbf{2.8} & 7758.8 & 3.8 & \textbf{2112.0} & \textbf{-} & 3415.9\\
quadrotor\_0 & window & window\_08\_v0 & \textbf{2.9} & 4623.0 & 3.4 & 7708.9 & 3.8 & \textbf{1657.6} & \textbf{-} & 2036.5\\
\bottomrule
\end{tabular}


==> results_tmp/tt_new.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
&  \multicolumn{3}{c}{idba*} & \multicolumn{3}{c}{sst} & \multicolumn{3}{c}{geo}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& icf & ilc & itf & scf & slc & stf & gcf & glc & gtf \\
\midrule
uni2\_0/kink\_0 & \textbf{19.8} & \textbf{17.7} & \textbf{1.1} & 99.0 & 99.0 & 40.1 & 32.2 & 19.3 & 2.0\\
uni2\_0/park & \textbf{5.8} & \textbf{5.8} & \textbf{0.2} & 99.0 & 99.0 & 40.1 & 5.9 & 5.9 & 0.3\\
uni2\_0/bugtrap\_0 & \textbf{27.2} & \textbf{25.1} & 2.2 & 99.0 & 99.0 & 40.1 & 33.9 & 28.4 & \textbf{2.0}\\
uni1\_0/park & 3.4 & 3.3 & 0.2 & 6.1 & 3.3 & \textbf{0.1} & \textbf{3.2} & \textbf{3.1} & 0.2\\
uni1\_0/bugtrap\_0 & \textbf{21.6} & \textbf{21.0} & 2.1 & 62.9 & 56.1 & \textbf{2.0} & 35.1 & 24.5 & 3.5\\
uni1\_0/kink\_0 & \textbf{21.1} & \textbf{13.3} & 1.4 & 49.2 & 32.9 & \textbf{0.4} & 25.0 & 14.0 & 1.2\\
uni1\_1/kink\_0 & \textbf{22.6} & \textbf{21.1} & \textbf{1.2} & 99.0 & 99.0 & 40.1 & 37.4 & 28.4 & 8.1\\
uni1\_2/wall\_0 & \textbf{18.9} & \textbf{18.1} & \textbf{0.8} & 41.1 & 41.1 & 31.7 & 99.0 & 99.0 & 40.1\\
car\_first\_order\_with\_1\_trailers\_0/kink\_0 & \textbf{16.5} & \textbf{16.7} & \textbf{4.8} & 59.6 & 58.3 & 9.6 & 39.5 & 35.6 & 13.2\\
car\_first\_order\_with\_1\_trailers\_0/bugtrap\_0 & \textbf{19.0} & \textbf{19.0} & 13.7 & 47.1 & 44.4 & \textbf{0.6} & 99.0 & 99.0 & 40.1\\
car\_first\_order\_with\_1\_trailers\_0/park & \textbf{4.8} & \textbf{4.8} & \textbf{1.0} & 99.0 & 99.0 & 40.1 & 6.0 & 6.0 & 1.2\\
quad2d/empty\_0 & 2.5 & \textbf{1.1} & 5.3 & 3.2 & 3.0 & 1.4 & \textbf{1.2} & 1.2 & \textbf{0.2}\\
quad2d/quad\_obs\_column & \textbf{5.3} & \textbf{3.6} & 6.8 & 99.0 & 99.0 & 40.1 & 10.1 & 4.0 & \textbf{4.8}\\
quad2d/quad2d\_recovery\_wo\_obs & \textbf{3.8} & \textbf{3.8} & \textbf{5.3} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
acrobot/swing\_up\_empty & \textbf{4.5} & \textbf{4.8} & \textbf{8.7} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
acrobot/swing\_down\_easy & \textbf{3.3} & \textbf{3.1} & \textbf{1.2} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
acrobot/swing\_down & \textbf{4.1} & \textbf{4.0} & \textbf{3.8} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
quadrotor\_0/empty\_0\_easy & 2.6 & 2.6 & 3.5 & 99.0 & 99.0 & 40.1 & \textbf{0.7} & \textbf{0.7} & \textbf{0.1}\\
quadrotor\_0/recovery & \textbf{2.6} & \textbf{2.6} & \textbf{5.5} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
quadrotor\_0/quad\_one\_obs & \textbf{3.2} & \textbf{3.4} & \textbf{17.9} & 99.0 & 99.0 & 40.1 & 99.0 & 99.0 & 40.1\\
\bottomrule
\end{tabular}


==> results_tmp2/merged_2023-10-01--20-29-41.tex.nice.tex <==
\begin{tabular}{lllrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{iDb-A*} & \multicolumn{4}{c}{SST*} & \multicolumn{4}{c}{RRT*+TO}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
 \# & System & Instance & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$\\
\midrule
0 & Acrobot & swing up & \textbf{1.0} & 7.6 & 5.3 & 4.7 & 0.4 & - & - & - & 0.7 & \textbf{4.2} & \textbf{4.4} & \textbf{4.0}\\
1 & Acrobot & swing obstacles 1 & \textbf{1.0} & 9.5 & \textbf{5.8} & 5.2 & 0.2 & - & - & - & \textbf{1.0} & \textbf{4.9} & 6.3 & \textbf{3.5}\\
2 & Car+Trailer & kink & \textbf{1.0} & 4.5 & \textbf{25.6} & \textbf{14.0} & \textbf{1.0} & \textbf{1.6} & 75.5 & 62.9 & \textbf{1.0} & 24.5 & 45.8 & 18.8\\
3 & Car+Trailer & park & \textbf{1.0} & \textbf{0.8} & \textbf{7.9} & \textbf{4.2} & 0.7 & 22.4 & 46.1 & 12.3 & 0.8 & 1.7 & 8.5 & 5.2\\
4 & Planar Rotor & hole & \textbf{0.9} & 31.6 & \textbf{3.6} & \textbf{3.0} & 0.8 & 101.0 & 10.2 & 7.7 & 0.8 & \textbf{19.3} & 4.2 & 3.5\\
5 & Planar Rotor & bugtrap & \textbf{1.0} & 29.9 & \textbf{5.2} & \textbf{5.2} & \textbf{1.0} & 42.1 & 11.8 & 8.7 & 0.8 & \textbf{13.2} & 11.7 & 10.5\\
6 & Rotor Pole & swing up obstacles & \textbf{1.0} & \textbf{7.3} & \textbf{4.0} & \textbf{3.9} & 0.0 & - & - & - & 0.4 & - & - & -\\
7 & Rotor Pole & small window & \textbf{1.0} & \textbf{10.5} & \textbf{4.5} & \textbf{4.5} & 0.0 & - & - & - & 0.4 & - & - & -\\
8 & Quadrotor v0 & recovery & \textbf{1.0} & \textbf{2.3} & \textbf{6.2} & \textbf{2.6} & 0.0 & - & - & - & 0.0 & - & - & -\\
9 & Quadrotor v0 & recovery obstacles & \textbf{1.0} & \textbf{3.9} & \textbf{5.3} & 3.5 & 0.0 & - & - & - & \textbf{1.0} & 8.4 & 7.3 & \textbf{3.4}\\
10 & Quadrotor v1 & obstacle & \textbf{1.0} & \textbf{2.7} & \textbf{2.7} & \textbf{2.4} & 0.1 & - & - & - & \textbf{1.0} & 3.3 & 4.7 & 3.6\\
11 & Quadrotor v1 & window & \textbf{1.0} & \textbf{4.0} & \textbf{2.6} & \textbf{2.2} & 0.3 & - & - & - & 0.8 & 29.2 & 6.3 & 2.9\\
12 & Unicycle 1 v0 & bugtrap & \textbf{1.0} & 3.2 & \textbf{22.3} & \textbf{20.7} & \textbf{1.0} & \textbf{0.3} & 70.2 & 24.3 & \textbf{1.0} & 6.8 & 45.6 & 23.9\\
13 & Unicycle 1 v2 & wall & \textbf{1.0} & 3.2 & \textbf{19.5} & \textbf{18.3} & \textbf{1.0} & \textbf{0.3} & 51.3 & 19.5 & 0.3 & - & - & -\\
14 & Unicycle 2 & bugtrap & \textbf{1.0} & 3.2 & \textbf{25.5} & \textbf{25.1} & \textbf{1.0} & \textbf{0.7} & 115.3 & 52.5 & \textbf{1.0} & 21.1 & 44.8 & 29.3\\
15 & Unicycle 2 & park & \textbf{1.0} & 0.4 & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.1} & 32.4 & 6.2 & 0.9 & 0.4 & 6.5 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp2/merged_2023-10-02--12-03-55.tex.nice.tex <==
\begin{tabular}{lllrrrrrrrrrrrr}
\toprule
& & &  \multicolumn{4}{c}{iDb-A*} & \multicolumn{4}{c}{SST*} & \multicolumn{4}{c}{RRT*+TO}\\
\cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-15}
 \# & System & Instance & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$ & $p$ & $t^{\textup{st}} [s]$ & $J^{\textup{st}}[s]$ & $J^{\textup{f}}[s]$\\
\midrule
0 & Acrobot & swing down & \textbf{1.0} & 15.2 & 5.2 & \textbf{3.2} & 0.0 & - & - & - & 0.9 & \textbf{2.3} & \textbf{4.0} & 4.0\\
1 & Acrobot & half swing down & \textbf{0.9} & \textbf{4.2} & \textbf{3.4} & \textbf{2.2} & 0.0 & - & - & - & 0.0 & - & - & -\\
2 & Acrobot & swing up & \textbf{1.0} & 7.6 & 5.3 & 4.7 & 0.4 & - & - & - & 0.7 & \textbf{4.2} & \textbf{4.4} & \textbf{4.0}\\
3 & Acrobot & swing up obstacles v0 & \textbf{1.0} & 8.3 & 6.2 & 4.5 & 0.3 & - & - & - & 0.8 & \textbf{5.1} & \textbf{5.4} & \textbf{3.6}\\
4 & Acrobot & swing obstacles 1 & \textbf{1.0} & 9.5 & \textbf{5.8} & 5.2 & 0.2 & - & - & - & \textbf{1.0} & \textbf{4.9} & 6.3 & \textbf{3.5}\\
5 & Car+Trailer & bugtrap & \textbf{1.0} & 2.6 & \textbf{19.2} & \textbf{19.0} & \textbf{1.0} & \textbf{0.9} & 73.3 & 48.3 & 0.1 & - & - & -\\
6 & Car+Trailer & kink & \textbf{1.0} & 4.5 & \textbf{25.6} & \textbf{14.0} & \textbf{1.0} & \textbf{1.6} & 75.5 & 62.9 & \textbf{1.0} & 24.5 & 45.8 & 18.8\\
7 & Car+Trailer & park & \textbf{1.0} & \textbf{0.8} & \textbf{7.9} & \textbf{4.2} & 0.7 & 22.4 & 46.1 & 12.3 & 0.8 & 1.7 & 8.5 & 5.2\\
8 & Planar Rotor & empty v0 & \textbf{1.0} & \textbf{0.1} & 1.1 & \textbf{1.0} & 0.9 & 1.5 & 1.9 & 1.1 & \textbf{1.0} & \textbf{0.1} & \textbf{1.0} & \textbf{1.0}\\
9 & Planar Rotor & empty v1 & \textbf{1.0} & 0.3 & 1.6 & \textbf{1.3} & \textbf{1.0} & 2.1 & 3.5 & 1.5 & \textbf{1.0} & \textbf{0.2} & \textbf{1.4} & 1.4\\
10 & Planar Rotor & hole & \textbf{0.9} & 31.6 & \textbf{3.6} & \textbf{3.0} & 0.8 & 101.0 & 10.2 & 7.7 & 0.8 & \textbf{19.3} & 4.2 & 3.5\\
11 & Planar Rotor & recovery obstacles & \textbf{1.0} & \textbf{7.6} & \textbf{4.7} & \textbf{4.4} & 0.0 & - & - & - & 0.4 & - & - & -\\
12 & Planar Rotor & recovery & \textbf{1.0} & \textbf{0.6} & \textbf{3.2} & \textbf{3.1} & 0.0 & - & - & - & 0.0 & - & - & -\\
13 & Planar Rotor & bugtrap & \textbf{1.0} & 29.9 & \textbf{5.2} & \textbf{5.2} & \textbf{1.0} & 42.1 & 11.8 & 8.7 & 0.8 & \textbf{13.2} & 11.7 & 10.5\\
14 & Planar Rotor & column & \textbf{1.0} & 2.6 & \textbf{3.4} & \textbf{3.3} & \textbf{1.0} & 33.5 & 11.1 & 7.3 & \textbf{1.0} & \textbf{2.3} & 8.7 & 3.5\\
15 & Rotor Pole & down & \textbf{1.0} & \textbf{2.7} & \textbf{3.9} & \textbf{3.2} & 0.0 & - & - & - & \textbf{1.0} & 11.1 & 5.7 & 5.7\\
16 & Rotor Pole & move v1 & \textbf{1.0} & \textbf{0.5} & 2.4 & 2.4 & 0.3 & - & - & - & \textbf{1.0} & 2.0 & \textbf{2.4} & \textbf{2.4}\\
17 & Rotor Pole & move v0 & \textbf{1.0} & 3.2 & 5.2 & 3.9 & 0.0 & - & - & - & \textbf{1.0} & \textbf{1.9} & \textbf{3.1} & \textbf{3.1}\\
18 & Rotor Pole & up & \textbf{1.0} & 26.1 & \textbf{3.9} & \textbf{3.2} & 0.0 & - & - & - & \textbf{1.0} & \textbf{6.2} & 4.4 & 4.4\\
19 & Rotor Pole & swing up obstacles & \textbf{1.0} & \textbf{7.3} & \textbf{4.0} & \textbf{3.9} & 0.0 & - & - & - & 0.4 & - & - & -\\
20 & Rotor Pole & window & \textbf{1.0} & \textbf{21.1} & \textbf{4.4} & \textbf{4.2} & 0.0 & - & - & - & 0.4 & - & - & -\\
21 & Rotor Pole & column & \textbf{1.0} & \textbf{31.7} & \textbf{4.1} & \textbf{3.2} & 0.0 & - & - & - & 0.2 & - & - & -\\
22 & Rotor Pole & small window & \textbf{1.0} & \textbf{10.5} & \textbf{4.5} & \textbf{4.5} & 0.0 & - & - & - & 0.4 & - & - & -\\
23 & Quadrotor v0 & empty v0 & \textbf{1.0} & 0.4 & 1.5 & 1.3 & 0.0 & - & - & - & \textbf{1.0} & \textbf{0.2} & \textbf{1.0} & \textbf{1.0}\\
24 & Quadrotor v0 & empty v1 & \textbf{1.0} & 1.2 & 2.3 & 1.4 & 0.0 & - & - & - & \textbf{1.0} & \textbf{0.3} & \textbf{1.2} & \textbf{1.2}\\
25 & Quadrotor v0 & obstacle & \textbf{1.0} & 4.6 & 6.6 & \textbf{3.2} & 0.0 & - & - & - & \textbf{1.0} & \textbf{3.4} & \textbf{5.5} & 3.7\\
26 & Quadrotor v0 & recovery & \textbf{1.0} & \textbf{2.3} & \textbf{6.2} & \textbf{2.6} & 0.0 & - & - & - & 0.0 & - & - & -\\
27 & Quadrotor v0 & recovery obstacles & \textbf{1.0} & \textbf{3.9} & \textbf{5.3} & 3.5 & 0.0 & - & - & - & \textbf{1.0} & 8.4 & 7.3 & \textbf{3.4}\\
28 & Quadrotor v0 & window & \textbf{1.0} & \textbf{6.4} & \textbf{4.4} & \textbf{2.4} & 0.0 & - & - & - & 0.9 & 28.3 & 7.0 & 2.9\\
29 & Quadrotor v1 & empty v0 & \textbf{1.0} & 0.3 & 0.9 & \textbf{0.8} & 0.8 & \textbf{0.1} & \textbf{0.8} & 0.8 & \textbf{1.0} & \textbf{0.1} & 1.0 & 1.0\\
30 & Quadrotor v1 & empty v1 & \textbf{1.0} & 0.3 & 1.3 & 1.0 & \textbf{1.0} & 1.2 & 3.9 & 2.0 & \textbf{1.0} & \textbf{0.2} & \textbf{0.9} & \textbf{0.9}\\
31 & Quadrotor v1 & obstacle & \textbf{1.0} & \textbf{2.7} & \textbf{2.7} & \textbf{2.4} & 0.1 & - & - & - & \textbf{1.0} & 3.3 & 4.7 & 3.6\\
32 & Quadrotor v1 & recovery & \textbf{1.0} & \textbf{0.7} & 2.2 & 2.1 & 0.0 & - & - & - & 0.8 & 1.4 & \textbf{2.0} & \textbf{2.0}\\
33 & Quadrotor v1 & recovery obstacles & \textbf{1.0} & \textbf{3.6} & \textbf{3.2} & 3.0 & 0.0 & - & - & - & \textbf{1.0} & 12.1 & 6.5 & \textbf{2.8}\\
34 & Quadrotor v1 & window & \textbf{1.0} & \textbf{4.0} & \textbf{2.6} & \textbf{2.2} & 0.3 & - & - & - & 0.8 & 29.2 & 6.3 & 2.9\\
35 & Unicycle 1 v0 & bugtrap & \textbf{1.0} & 3.2 & \textbf{22.3} & \textbf{20.7} & \textbf{1.0} & \textbf{0.3} & 70.2 & 24.3 & \textbf{1.0} & 6.8 & 45.6 & 23.9\\
36 & Unicycle 1 v0 & kink & \textbf{1.0} & 2.7 & \textbf{21.4} & \textbf{13.2} & \textbf{1.0} & \textbf{0.1} & 58.8 & 15.5 & \textbf{1.0} & 2.5 & 25.9 & 14.1\\
37 & Unicycle 1 v0 & park & \textbf{1.0} & 0.4 & 3.6 & \textbf{3.1} & \textbf{1.0} & \textbf{0.1} & 10.9 & \textbf{3.1} & \textbf{1.0} & \textbf{0.1} & \textbf{3.5} & \textbf{3.1}\\
38 & unicycle1\_v1 & kink & \textbf{1.0} & \textbf{2.4} & \textbf{23.9} & \textbf{21.1} & \textbf{1.0} & 14.9 & 44.5 & 24.5 & \textbf{1.0} & 11.1 & 49.3 & 25.4\\
39 & Unicycle 1 v2 & wall & \textbf{1.0} & 3.2 & \textbf{19.5} & \textbf{18.3} & \textbf{1.0} & \textbf{0.3} & 51.3 & 19.5 & 0.3 & - & - & -\\
40 & Unicycle 2 & bugtrap & \textbf{1.0} & 3.2 & \textbf{25.5} & \textbf{25.1} & \textbf{1.0} & \textbf{0.7} & 115.3 & 52.5 & \textbf{1.0} & 21.1 & 44.8 & 29.3\\
41 & Unicycle 2 & kink & \textbf{1.0} & \textbf{2.2} & \textbf{19.4} & \textbf{17.7} & \textbf{1.0} & 2.3 & 96.2 & 40.6 & \textbf{1.0} & 4.6 & 37.3 & 18.3\\
42 & Unicycle 2 & park & \textbf{1.0} & 0.4 & \textbf{5.8} & \textbf{5.8} & \textbf{1.0} & \textbf{0.1} & 32.4 & 6.2 & 0.9 & 0.4 & 6.5 & \textbf{5.8}\\
\bottomrule
\end{tabular}


==> results_tmp2/summary_search_2023-10-02--13-06-23.tex <==
\begin{tabular}{llcccccc}
\toprule
 & &   \multicolumn{2}{c}{Euclidean} & \multicolumn{2}{c}{Roadmap} & \multicolumn{2}{c}{Blind} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 Dynamics & Instance & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t [s] & n  { \scriptsize $[\cdot 10^3]$ } & t [s]\\
\midrule
Car+Trailer & bugtrap & 12.5 & 0.7 & \textbf{6.3} & \textbf{0.3} & 24.6 & 1.3\\
Planar Rotor & bugtrap & 125.5 & 15.7 & \textbf{51.0} & \textbf{5.5} & - & -\\
Rotor Pole & window & 53.6 & \textbf{11.0} & \textbf{40.8} & 11.6 & 81.1 & 15.1\\
Quadrotor v0 & obstacle & 74.5 & 16.3 & \textbf{36.7} & \textbf{10.4} & - & -\\
Quadrotor v0 & recovery obstacles & 8.9 & \textbf{1.4} & \textbf{6.5} & 3.4 & 47.5 & 12.3\\
Quadrotor v1 & window & 20.4 & \textbf{2.8} & \textbf{17.0} & 9.4 & 69.5 & 19.0\\
Unicycle 1 v0 & bugtrap & 18.2 & 2.1 & \textbf{6.2} & \textbf{0.9} & 27.5 & 2.8\\
Unicycle 2 & bugtrap & 74.2 & 9.1 & \textbf{41.6} & \textbf{5.8} & 84.6 & 10.1\\
\bottomrule
\end{tabular}

